Rosita++: Automatic Higher-Order Leakage Elimination from Cryptographic Code

Side-channel attacks are a major threat to the security of cryptographic implementations, particularly for small devices that are under the physical control of the adversary. While several strategies for protecting against side-channel attacks exist, these often fail in practice due to unintended interactions between values deep within the CPU. To detect and protect from side-channel attacks, several automated tools have recently been proposed; one of their common limitations is that they only support first-order leakage. In this work, we present the first automated tool for detecting and eliminating higher-order leakage from cryptographic implementations. Rosita++ proposes statistical and software-based tools to allow high-performance higher-order leakage detection. It then uses the code rewrite engine of Rosita (Shelton et al. NDSS 2021) to eliminate detected leakage. For the sake of practicality we evaluate Rosita++ against second and third order leakage, but our framework is not restricted to only these orders. We evaluate Rosita++ against second-order leakage with three-share implementations of two ciphers, PRESENT and Xoodoo, and with the second-order Boolean-to-arithmetic masking, a core building block of masked implementations of many cryptographic primitives, including SHA-2, ChaCha and Blake. We show effective second-order leakage elimination at a performance cost of 36% for Xoodoo, 189% for PRESENT, and 29% for the Boolean-to-arithmetic masking. For third-order analysis, we evaluate Rosita++ against the third-order leakage using a four-share synthetic example that corresponds to typical four-share processing. Rosita++ correctly identified this leakage and applied code fixes.

==> Makefile <==
# Generic paper Makefile
#
# For usage hints, "make help"
#
#  To create a LaTeX diff against the hg "tip" revision, use the target
#  "diff" (or "viewdiff").
#  To use a revision other than "tip", speciff DIFF=x on the 
#  make command line to choose the revision x.
#

# Verbosity
ifeq (${V},1)
Q:=
else
Q:=@
endif

export max_print_line=1000
export error_line=254
export half_error_line=238

.PHONY: all

BIBDIR     ?= /home/disy/lib/BibTeX:../../../bibtex:../bibtex
LaTeXEnv   = TEXINPUTS=".:/home/disy/lib/TeX:/home/disy/lib/ps:${TEXINPUTS}:"
BibTexEnv  = BIBINPUTS=".:${BIBDIR}:${BIBINPUTS}:"
BibFiles   = defs-abbrev,extra,combined,systems,fm,other

LaTeX      = ${LaTeXEnv} pdflatex -interaction=nonstopmode
LaTeXdiff  = ./tools/latexdiff
BibTeX     = ${BibTexEnv} bibtex
Fig2Eps    = fig2dev -L eps
Dia2Eps    = dia -t eps -e
AS         = $(shell which as)
CC         = $(shell which gcc)
GnuPlot	   = gnuplot
Inkscape   = $(shell which inkscape)
Eps2Pdf	   = epstopdf --outfile
PdfView	   = xpdf
Pdf2Ps	   = pdf2ps
RmCR       = tr -d '\r'
sed        = $(shell which sed)
#PdfView    = open -a preview
#PdfView    = acroread 
Lpr 	   = lpr
mv	   = mv
awk	   = awk
R	   = R

# Use either "report" or "paper", depending on the template.
# To add a further target, simply append the basename of the .tex file here
Targets    = horosita
SRCS = horosita.tex # methodology.tex


# CONFIGURATION OPTIONS
# =====================

# For ACM SIG camera ready submission. This will only work if Target
# is a single identifier. You should then be able to use the "camera" target,
# after setting CamRoot appropriately. Answer "no" for re-making references.bib
# Set CamRoot as the filename root per publisher's instructions.
# Should be <paperno>-<lastname-of-first-author>
CamRoot    = <paperno>-<last>
CamDir	   = cameraready

# Any other stuff that may be needed

# END CONFIGURATION OPTIONS
# =========================

Optional = $(addsuffix -diff, $(Targets))
All = $(Targets) $(Optional)
Diffopts= #--type=BWUNDERLINE #-c .latexdiffconfig --append-safecmd="Comment"

Gnuplot_Sources = $(wildcard figures/*.gnuplot)
Figures = $(Gnuplot_Sources:.gnuplot=.pdf)



Pdf = $(addsuffix .pdf, $(Targets))
Tex = $(addsuffix .tex, $(Targets))
Diff_Pdf = $(addsuffix .pdf, $(Optional))

.PHONY: FORCE

all: pdf
diff: diff_pdf
FORCE: pdf
ps: $(Ps)
pdf: $(Figures) Makefile $(Pdf)
diff_pdf: $(Figures) Makefile $(Diff_Pdf)

%.pdf: %.perf tools/bargraph.pl
	@echo $< '->' $@
	${Q} ${BarGraph} -pdf $< > $@

%.pdf: %.eps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.pdf: %.ps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

#%.eps: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -E $@ > /dev/null 2>&1

#%.pdf: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -A $@ > /dev/null 2>&1

# This target allows you to add figures which have the extension .c_pp that
# correspond to .c sources. Your .c sources can use the lines '/*<*/' and
# '/*>*/' to surround parts of the source you don't want shown in your PDF.
# This allows you to write a .c file that can be compile-checked here and then
# remove extraneous lines for display.
%.c_pp: %.c
	@echo $< '->' $@
	${Q}$(if ${CC},${CC} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.s_pp: %.s
	@echo $< '->' $@
	${Q}$(if ${AS},${AS} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.eps: %.dia
	@echo $< '->' $@
	${Q} ${Dia2Eps} $@ $<

%.eps: %.fig
	@echo $< '->' $@
	${Q} ${Fig2Eps} $< $@

%.eps: %.gnuplot
	@echo $< '->' $@
	${Q} ${GnuPlot} $<

%.eps: %.r
	@echo $< '->' $@
	${Q} ${R} --vanilla < $<

%.pdf: %.pdf-shipped
	cp $< $@

view: pdf
	${Q}for i in $(Pdf); do \
		$(PdfView) $$i & \
	done

viewdiff: diff
	${Q}for i in $(Diff_Pdf); do \
		$(PdfView) $$i & \
	done

print: pdf
	${Q}for i in $(Pdf); do \
		$(Lpr) $$i \
	done

clean:
	rm -f *.aux *.toc *.bbl *.blg *.dvi *.log *.pstex* *.eps *.cb *.brf \
		*.idx *.out *.ps *-diff.* *.mps .log *.diff horosita.pdf

help:
	@echo "Main targets: all diff camera view viewdiff print clean realclean tar"
	@echo "'make diff' will show changes to head revision"
	@echo "'make DIFF=<rev> diff' will show changes to revision <rev>"
	@echo "Avoid TeX \def with arguments, this breaks latexdiff (use \newcommand)"


##############################################################################

DIFF ?= tip

%-diff.dvi: %-diff.tex

%-diff.tex: %.tex FORCE
	@echo "====> Retrieving revision $(DIFF) of $<"
	hg cat -r $(DIFF) $<  > $(@:-diff.tex=-$(DIFF)-diff.tex)
	@echo "====> Creating diff of revision $(DIFF) of $<"
	$(LaTeXdiff) $(Diffopts) $(@:-diff.tex=-$(DIFF)-diff.tex) $< | \
	${RmCR} > $@

.PHONY: FORCE
FORCE:

# don't delete %.aux intermediates
.SECONDARY:

##############################################################################

Rerun = '(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)'
Rerun_Bib = 'No file.*\.bbl|Citation.*undefined'
Undefined = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
Error = '^! '

horosita-small.pdf: horosita.pdf
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/ebook -dNOPAUSE -dQUIET -dBATCH -sOutputFile=horosita-small.pdf horosita.pdf

horosita.pdf: horosita.tex  $(Figures) Makefile ${SRCS}
	${Q}if ! test -e horosita.bbl || test horosita.bib -nt horosita.bbl; then rm -f horosita.bbl; fi
	@echo "====> LaTeX first pass: $(<)"
	${Q}$(LaTeX) $< >.log || if egrep -q $(Error) horosita.log ; then cat .log; rm $@; false ; fi
	${Q}if egrep -q $(Rerun_Bib) horosita.log ; then echo "====> BibTex" && ( $(BibTeX) horosita > .log || ( cat .log ; false ) ) && echo "====> LaTeX BibTeX pass" && $(LaTeX) >.log $< || if egrep -q $(Error) horosita.log ; then cat .log; rm $@; false ; fi ; fi
	${Q}if egrep -q $(Rerun) horosita.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) horosita.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) horosita.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if [ -a .NeedGS ]; then gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=tmp.pdf $@; mv tmp.pdf $@; fi
	@echo "====> Undefined references and citations in $(<):"
	@egrep -i $(Undefined) horosita.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" horosita.log || echo "None."

##############################################################################
# Generate a list of FIXMEs 
fixmes: 
	${Q}for i in $(Tex); do \
		echo "FIXMEs in $$i:"; \
		nl -b a $$i | grep "FIXME{" | nl -b a; \
		echo -n "Total FIXMES: " && grep "FIXME{" $$i | wc -l; \
		echo; \
	done

usb.pdf: dtrt.sty

